Analog electronics for beam instrumentation

The task of analog front-end electronics in beam instrumentation is to optimize the useful information content of the signal delivered by an instrument. It must suppress signal components that do not contribute to the measured quantity. It must filter to put bounds on bandwidth and possibly dynamic range, to relax the demands made of subsequent processing stages. It must minimize noise, reject interference and match the signal to transmission media and digital acquisition equipment. Since the circuitry must often operate in radio-active areas, the accent is on passive electronics.

==> makefile <==
SOURCE = abstract.tex conclusion.tex emc.tex filters.tex introduction.tex noise.tex radhard.tex	tdr.tex	\
tlines.tex tltransformers.tex bib.tex
       

belleman.pdf: belleman.tex $(SOURCE)
	latexmk	-pdfdvi	$<


clean:
	latexmk	-c -quiet
	rm -f Old.*	       

distclean:
	latexmk	-C -quiet
	rm -f Old.*

